Accelerating Verified-Compiler Development with a Verified Rewriting Engine

Compilers are a prime target for formal verification, since compiler bugs invalidate higher-level correctness guarantees, but compiler changes may become more labor-intensive to implement, if they must come with proof patches. One appealing approach is to present compilers as sets of algebraic rewrite rules, which a generic engine can apply efficiently. Now each rewrite rule can be proved separately, with no need to revisit past proofs for other parts of the compiler. We present the first realization of this idea, in the form of a framework for the Coq proof assistant. Our new Coq command takes normal proved theorems and combines them automatically into fast compilers with proofs. We applied our framework to improve the Fiat Cryptography toolchain for generating cryptographic arithmetic, producing an extracted command-line compiler that is about 1000$\times$ faster while actually featuring simpler compiler-specific proofs.

==> Makefile <==
.PHONY: cache all clean zip remake-patch

all: bcprules.sty rewriting.tex rewriting.bib
	sed -i 's/frozencache=false/frozencache/g' rewriting.tex
	pdflatex rewriting.tex
	bibtex rewriting.aux
	pdflatex rewriting.tex
	pdflatex rewriting.tex

cache: bcprules.sty
	sed -i 's/frozencache/frozencache=false/g; s/frozencache=false=false/frozencache=false/g' rewriting.tex
	pdflatex -shell-escape rewriting.tex

error_missing_file = $(error Missing original file $(1)!  If you downloaded this from the arXiv, pass IGNORE_MISSING_ORIGINALS=1 to suppress this message.)

IGNORE_MISSING_ORIGINALS?=
ifneq (,$(wildcard ../rewriting.tex))
rewriting.tex: ../rewriting.tex diff.patch
	cp ../rewriting.tex $@ && patch -p3 $@ diff.patch
else
ifneq (1,$(IGNORE_MISSING_ORIGINALS))
$(call error_missing_file,../rewriting.tex)
endif
endif

ifneq (,$(wildcard ../rewriting.bib))
rewriting.bib : % : ../%
	cp $< $@
else
ifneq (1,$(IGNORE_MISSING_ORIGINALS))
$(call error_missing_file,../rewriting.bib)
endif
endif

remake-patch:
	{ diff -Naur ../rewriting.tex rewriting.tex; true; } > diff.patch

clean::
	rm -rf *~ \#* rewriting-for-split.tex rewriting.pdf *.pyg *.out *.aux *.auxlock *.log *.vtc *.blg _minted-rewriting-for-split/ rewriting-for-split.appendix.startpage *.dep *.dpth rewriting-for-split.supplement.onlyendpage rewriting-for-split.supplement.onlystartpage rewriting-main.pdf
	rm -f rewriting.appendix.startpage rewriting.supplement.onlyendpage rewriting.supplement.onlystartpage rewriting.supplement.startpage
	# bcprules.sty
	# rewriting-for-split.supplement.startpage rewriting-for-split.pdf

zip: clean
	rm -f ../arxiv.zip
	zip -r ../arxiv.zip .

bcprules.sty: ../bcprules.sty
	cp $< $@

.PHONY: update-minted download-minted clean-minted make-minted
download-minted:
	wget https://mirrors.ctan.org/macros/latex/contrib/minted.zip
	wget https://mirrors.ctan.org/macros/latex/contrib/latex2pydata.zip
	wget https://mirrors.ctan.org/macros/latex/contrib/fvextra.zip
	unzip minted.zip
	unzip latex2pydata.zip
	unzip fvextra.zip

clean-minted:
	rm -rf minted minted.zip
	rm -rf latex2pydata latex2pydata.zip
	rm -rf fvextra fvextra.zip

make-minted:
	cd minted && tex minted.ins
	cp minted/*.sty ./
	cd latex2pydata && tex latex2pydata.ins
	cp latex2pydata/*.sty ./
	cd fvextra && tex fvextra.ins
	cp fvextra/*.sty ./

update-minted:
	$(MAKE) download-minted
	$(MAKE) make-minted
	$(MAKE) clean-minted
